Open Photoacoustic Cell for Blood Sugar Measurement: Numerical Calculation of Frequency Response

A new approach for continuous and non-invasive monitoring of the glucose concentration in human epidermis has been suggested recently. This method is based on photoacoustic (PA) analysis of human interstitial fluid. The measurement can be performed in vitro and in vivo and, therefore, may form the basis for a non-invasive monitoring of the blood sugar level for diabetes patients. It requires a windowless PA cell with an additional opening that is pressed onto the human skin. Since signals are weak, advantage is taken of acoustic resonances of the cell. Recently, a numerical approach based on the Finite Element (FE) Method has been successfully used for the calculation of the frequency response function of closed PA cells. This method has now been adapted to obtain the frequency response of the open cell. Despite the fact that loss due to sound radiation at the opening is not included, fairly good accordance with measurement is achieved.

==> Vorspann.tex <==
%\documentclass[10pt,a4paper]{article}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}

%\usepackage{german}
\usepackage[latin1]{inputenc}
\usepackage{latexsym} % vgl. Kopka, p121
\usepackage{graphicx}
\usepackage{psfrag}
\usepackage{exscale}
\usepackage[permil]{overpic}       % zum berlagern von TeX-Ausdrcken und EPS-Bildern
\usepackage[vflt]{floatflt}        % Text umflie§t Grafiken und Tabellen
\usepackage{times}
\usepackage{makeidx}               % Anlegen eines Registers
%\usepackage{sidecap}     % seitliche Anordnung der figure-captions
\usepackage{color}
\usepackage{framed,color}
\usepackage{hyperref}


\makeindex   % Anlegen eines Registers

%\pagestyle{headings}
%\markright{Baumann: FE und Technische Physik}

%\pagestyle{myheadings}
%\markboth{B. Baumann, HAW Hamburg}{Finite Elemente und Technische Physik}

\renewcommand{\familydefault}{cmss}
\newfont{\Head}{cmss17 at 36pt}
\newfont{\head}{cmss17}
%\newfont{\authorfont}{cmss10 at 20.74pt}
\newfont{\auflage}{cmss10 at 14.4pt}
%\newfont{\fuit}{cmfi10 at 48pt}
%\newfont{\dunh}{cmdunh10 at 12pt}
\input epsf % defines \epsfbox and supporting macros
\epsfverbosetrue % messages will show height and width of figures

%\setlength{\textheight}{190mm}    % C5-Format (liefert richtiges
%                                   % Lngen- zu Breitenverhltnis)
% 
%\setlength{\topmargin}{0mm}       % Vorgabe von PRZIS DRUCK
%\setlength{\oddsidemargin}{0mm}   % Vorgabe von PRZIS DRUCK
%\setlength{\evensidemargin}{0mm}  % Vorgabe von PRZIS DRUCK

\newenvironment{dsc}[1]      % Description-Umgebung ohne Einzug
   {\begin{list}{}{%           (vgl Kopka, p200f)
      \settowidth{\labelwidth}{\textbf{#1}}
      \setlength{\leftmargin}{\labelwidth}
         \addtolength{\leftmargin}{\labelsep}
      \setlength{\parsep}{0.5ex plus0.2ex minus0.2ex}
      \setlength{\itemsep}{0.3ex}
      \renewcommand{\makelabel}[1]{\textbf{##1}\hfill}}}
   {\end{list}}

\newcounter{AfgNr}   % Fr die Aufgabennummerierung
\newcounter{AuxVar}  % Hilfsvariable
\newcounter{AuxVar1} % Hilfsvariable

%\DeclareMathOperator{\Tr}{Tr}
                                           
\newcommand{\impl}{\quad\Rightarrow\quad} % Impliziert-Pfeil

\newcommand{\pg}[2]{$#1\;{\rm#2}$} % Zur Darstellung phys. Gr§en m. 
                                   % Ma§zahl und Ma§einheit

\newcommand{\pgz}[3]{$#1\cdot 10^{#2}\;{\rm#3}$} % Zur Darstellung phys. Gr§en m. 
                                   % Ma§zahl einschl. Zehnerpotenz und Ma§einheit

\newcommand{\ze}[2]{#1\;{\rm#2}} % neue Version von \pg
                                 % Ma§Zahl mal Ma§Einheit

\newcommand{\zze}[3]{#1\cdot 10^{#2}\;{\rm#3}} % neue Version von \pgz
                                   % Ma§Zahl mal Zehnerpotenz mal Ma§Einheit

\newfont{\tensy}{cmsy10}           % Zur Darstellung chem. Formeln                          
\newcommand{\cf}[1]{{$\fontdimen16\tensy=3.0pt
                      \fontdimen17\tensy=3.0pt
                      \mathrm{#1}$}}   

\def\acrobat{\hyperdef{jump}{here}{}}

\newcommand{\ce}[3]{{$^{#1}_{#2}\mathrm{#3}$}}  % Zur Darstellung chem. Elemente 

\newcommand{\Lsg}{\newline{\sl Lsung:}} % Zur Darstellung von 
                                         % Lsungen nach Aufgaben
                                         
\newcommand{\grad}{^\circ} % Winkel in Grad                                        
                                        
\newcommand{\fm}[1] % Formel
{\begin{displaymath}#1\end{displaymath}}

\newcommand{\nfm}[1] % numerierte Formel
{\begin{equation}#1\end{equation}}

\newcommand{\nmzfm}[1] % numerierte mehrzeilige Formel
{\begin{eqnarray}#1\end{eqnarray}}

\newcommand{\mzfm}[1] % mehrzeilige Formel
{\begin{eqnarray*}#1\end{eqnarray*}}

\newcommand{\gfm}[1] % gerahmte Formel
{\begin{displaymath}\fbox{$\displaystyle #1$}\end{displaymath}}

\newcommand{\ngfm}[1] % gerahmte und numerierte Formel
{\begin{equation}\fbox{$\displaystyle #1$}\end{equation}}

\newcommand{\mzgfm}[1] % mehrzeilige gerahmte Formel
{\begin{displaymath}\fbox{$\begin{array}{rcl} #1\end{array}$}\end{displaymath}}

\newcommand{\figcapt}[2] % genderte Bildunterschriften
{\renewcommand{\normalsize}{\small}\textbf{\caption[#1]{\textmd{#2}}}}

\newcommand{\fif}[1] % fett in Formeln
{\mathbf{#1}}
%{\mbox{\boldmath$#1$}}

\newcommand{\bi}[4] % bestimmtes Integral
{\int_{#1}^{#2}{#3}\,{#4}}

\newcommand{\ubi}[2] % unbestimmtes Integral
{\int{#1}\,{#2}}

\renewcommand{\labelitemi}{$\triangleright$}

\renewcommand{\indexname}{Sachverzeichnis} % vgl. german.sty

%\renewcommand{\bibname}{Literatur} % vgl. german.sty

\definecolor{shadecolor}{gray}{.90} % Hintergrundfarbe (0.90 ist ein 
                                    % guter Wert)

%\newtheorem{beispielc}{Beispiel}[chapter] % Beispiel mit Kapitelnumerierung
\newcommand{\gBeispielc}[1]
{\begin{shaded}\begin{beispielc}\upshape #1\end{beispielc}\end{shaded}}

\newtheorem{beispiels}{Beispiel}[section] % Beispiel mit Abschnittnumerierung
\newcommand{\Beispiel}[1]
{\begin{shaded}\begin{beispiels}\upshape #1\end{beispiels}\end{shaded}}

%\newtheorem{aufgabe}{Aufgabe}[chapter]
\newcommand{\Aufgabe}[1]
{\begin{aufgabe}\normalfont{#1}\end{aufgabe}}

\newtheorem{aufgabeS}{Aufgabe}[section]
\newcommand{\AufgabeS}[1]
{\begin{aufgabeS}\normalfont{#1}\end{aufgabeS}}

\newcommand{\qM} % quadratische Matrix
{\left[\ddots\right]}

\newcommand{\SV} % Spaltenvektor
{\left[\vdots\right]}

\newcommand{\Tensoreps}[0]
{\begin{picture}(6,8)
	\put(0,5.4){\tiny$\leftrightarrow$}
	\put(0,0){$\epsilon$}
\end{picture}}

\newcommand{\Tensore}[0]
{\begin{picture}(7,8)
	\put(0,7.9){\tiny$\rightarrow$}
	\put(0,5.4){\tiny$\leftrightarrow$}
	\put(0,0){$e$}
\end{picture}}

\newcommand{\Tensorvareps}[0]
{\begin{picture}(6,8)
	\put(0,5.4){\tiny$\leftrightarrow$}
	\put(0,0){$\varepsilon$}
\end{picture}}

\newcommand{\Tensorsig}[0]
{\begin{picture}(6,8)
	\put(0,5.4){\tiny$\leftrightarrow$}
	\put(0,0){$\sigma$}
\end{picture}}

\newcommand{\TensorNull}[0]
{\begin{picture}(9,10)
	\put(-1,8.2){\tiny$\leftrightarrow$}
	\put(0,0){$0$}
\end{picture}}

\newcommand{\TensorC}[0]
{\begin{picture}(9,10)
	\put(1,10.9){\tiny$\leftrightarrow$}
	\put(1,8.4){\tiny$\leftrightarrow$}
	\put(0,0){$C$}
\end{picture}}

\newcommand{\Hfa}[1]
{\setlength{\unitlength}{0.1mm}
\begin{picture}(50,75)
 	\put(0,0){\line(0,1){40}}
	\put(36,0){\line(0,1){45}}
 	\put(0,36){\line(1,-1){36}}
	\qbezier(0,40)(18,50)(36,45)
	\put(30,-25){\scriptsize$#1$}
\end{picture}}

\newcommand{\Hfb}[1]
{\setlength{\unitlength}{0.1mm}
\begin{picture}(50,50)
	\put(0,0){\line(0,1){40}}
	\put(36,0){\line(0,1){45}}
	\put(0,0){\line(1,1){36}}
	\qbezier(0,40)(18,50)(36,45)
	\put(30,-25){\scriptsize$#1$}
\end{picture}}

\newcommand{\HHa}[1]
{\setlength{\unitlength}{0.1mm}
\begin{picture}(50,50)
	\put(0,0){\line(0,1){40}}
	\put(36,0){\line(0,1){40}}
	\put(0,0){\line(1,1){36}}
	\put(0,36){\line(1,-1){36}}
	\put(30,-25){\scriptsize$#1$}	
\end{picture}}

\newcommand{\HHb}[1]
{\setlength{\unitlength}{0.1mm}
\begin{picture}(50,50)
	\put(0,0){\line(0,1){40}}
	\put(36,0){\line(0,1){40}}
	\put(0,36){\line(1,-1){36}}
	\put(0,40){\line(1,-1){36}}
	\put(30,-25){\scriptsize$#1$}	
\end{picture}}

\newcommand{\HHc}[1]
{\setlength{\unitlength}{0.1mm}
\begin{picture}(50,50)
	\put(0,0){\line(0,1){40}}
	\put(36,0){\line(0,1){40}}
	\put(0,0){\line(1,1){36}}
	\put(0,4){\line(1,1){36}}
	\put(30,-25){\scriptsize$#1$}	
\end{picture}}

\newcommand{\Hfnull}[4]
{\setlength{\unitlength}{0.1mm}
\begin{picture}(110,55)
	\qbezier(0,15)(40,50)(108,40)
	\put(0,0){\circle{5}}
	\put(36,0){\circle{5}}
	\put(72,0){\circle{5}}
	\put(108,0){\circle{5}}
	\put(0,36){\line(1,-1){36}}
	\put(36,0){\line(1,0){36}}
	\put(72,0){\line(1,0){36}}
	\put(-6,-25){\scriptsize$#1$}
	\put(30,-25){\scriptsize$#2$}
	\put(66,-25){\scriptsize$#3$}
	\put(102,-25){\scriptsize$#4$}
\end{picture}}

\newcommand{\Hfeins}[4]
{\setlength{\unitlength}{0.1mm}
\begin{picture}(110,55)
	\qbezier(0,15)(40,50)(108,40)
	\put(0,0){\circle{5}}
	\put(36,0){\circle{5}}
	\put(72,0){\circle{5}}
	\put(108,0){\circle{5}}
	\put(0,0){\line(1,1){36}}
	\put(36,36){\line(1,-1){36}}
	\put(72,0){\line(1,0){36}}
	\put(-6,-25){\scriptsize$#1$}
	\put(30,-25){\scriptsize$#2$}
	\put(66,-25){\scriptsize$#3$}
	\put(102,-25){\scriptsize$#4$}
\end{picture}}

\newcommand{\Hfzwei}[4]
{\setlength{\unitlength}{0.1mm}
\begin{picture}(110,55)
	\qbezier(0,15)(40,50)(108,40)
	\put(0,0){\circle{5}}
	\put(36,0){\circle{5}}
	\put(72,0){\circle{5}}
	\put(108,0){\circle{5}}
	\put(0,0){\line(1,0){36}}
	\put(36,0){\line(1,1){36}}
	\put(72,36){\line(1,-1){36}}
	\put(-6,-25){\scriptsize$#1$}
	\put(30,-25){\scriptsize$#2$}
	\put(66,-25){\scriptsize$#3$}
	\put(102,-25){\scriptsize$#4$}
\end{picture}}

\newcommand{\Hfdrei}[4]
{\setlength{\unitlength}{0.1mm}
\begin{picture}(110,55)
	\qbezier(0,15)(40,50)(108,40)
	\put(0,0){\circle{5}}
	\put(36,0){\circle{5}}
	\put(72,0){\circle{5}}
	\put(108,0){\circle{5}}
	\put(0,0){\line(1,0){36}}
	\put(36,0){\line(1,0){36}}
	\put(72,0){\line(1,1){36}}
	\put(-6,-25){\scriptsize$#1$}
	\put(30,-25){\scriptsize$#2$}
	\put(66,-25){\scriptsize$#3$}
	\put(102,-25){\scriptsize$#4$}
\end{picture}}

\newcommand{\HnullHnull}[4]
{\setlength{\unitlength}{0.1mm}
\begin{picture}(110,55)
	\put(0,0){\circle{5}}
	\put(36,0){\circle{5}}
	\put(72,0){\circle{5}}
	\put(108,0){\circle{5}}
	\put(0,36){\line(1,-1){36}}
	\put(36,0){\line(1,0){36}}
	\put(72,0){\line(1,0){36}}
	\put(0,40){\line(1,-1){36}}
	\put(36,4){\line(1,0){36}}
	\put(72,4){\line(1,0){36}}
	\put(-6,-25){\scriptsize$#1$}
	\put(30,-25){\scriptsize$#2$}
	\put(66,-25){\scriptsize$#3$}
	\put(102,-25){\scriptsize$#4$}
\end{picture}}

\newcommand{\HnullHeins}[4]
{\setlength{\unitlength}{0.1mm}
\begin{picture}(110,55)
	\put(0,0){\circle{5}}
	\put(36,0){\circle{5}}
	\put(72,0){\circle{5}}
	\put(108,0){\circle{5}}
	\put(0,36){\line(1,-1){36}}
	\put(36,0){\line(1,0){36}}
	\put(72,0){\line(1,0){36}}
	\put(0,4){\line(1,1){36}}
	\put(36,40){\line(1,-1){36}}
	\put(72,4){\line(1,0){36}}
	\put(-6,-25){\scriptsize$#1$}
	\put(30,-25){\scriptsize$#2$}
	\put(66,-25){\scriptsize$#3$}
	\put(102,-25){\scriptsize$#4$}
\end{picture}}

\newcommand{\HnullHzwei}[4]
{\setlength{\unitlength}{0.1mm}
\begin{picture}(110,55)
	\put(0,0){\circle{5}}
	\put(36,0){\circle{5}}
	\put(72,0){\circle{5}}
	\put(108,0){\circle{5}}
	\put(0,36){\line(1,-1){36}}
	\put(36,0){\line(1,0){36}}
	\put(72,0){\line(1,0){36}}
	\put(0,4){\line(1,0){36}}
	\put(36,4){\line(1,1){36}}
	\put(72,40){\line(1,-1){36}}
	\put(-6,-25){\scriptsize$#1$}
	\put(30,-25){\scriptsize$#2$}
	\put(66,-25){\scriptsize$#3$}
	\put(102,-25){\scriptsize$#4$}
\end{picture}}

\newcommand{\HeinsHeins}[4]
{\setlength{\unitlength}{0.1mm}
\begin{picture}(110,55)
	\put(0,0){\circle{5}}
	\put(36,0){\circle{5}}
	\put(72,0){\circle{5}}
	\put(108,0){\circle{5}}
	\put(0,0){\line(1,1){36}}
	\put(36,36){\line(1,-1){36}}
	\put(72,0){\line(1,0){36}}
	\put(0,4){\line(1,1){36}}
	\put(36,40){\line(1,-1){36}}
	\put(72,4){\line(1,0){36}}
	\put(-6,-25){\scriptsize$#1$}
	\put(30,-25){\scriptsize$#2$}
	\put(66,-25){\scriptsize$#3$}
	\put(102,-25){\scriptsize$#4$}
\end{picture}}

\newcommand{\HeinsHzwei}[4]
{\setlength{\unitlength}{0.1mm}
\begin{picture}(110,55)
	\put(0,0){\circle{5}}
	\put(36,0){\circle{5}}
	\put(72,0){\circle{5}}
	\put(108,0){\circle{5}}
	\put(0,0){\line(1,1){36}}
	\put(36,36){\line(1,-1){36}}
	\put(72,0){\line(1,0){36}}
	\put(0,4){\line(1,0){36}}
	\put(36,4){\line(1,1){36}}
	\put(72,40){\line(1,-1){36}}
	\put(-6,-25){\scriptsize$#1$}
	\put(30,-25){\scriptsize$#2$}
	\put(66,-25){\scriptsize$#3$}
	\put(102,-25){\scriptsize$#4$}
\end{picture}}

\newcommand{\HzweiHzwei}[4]
{\setlength{\unitlength}{0.1mm}
\begin{picture}(110,55)
	\put(0,0){\circle{5}}
	\put(36,0){\circle{5}}
	\put(72,0){\circle{5}}
	\put(108,0){\circle{5}}
	\put(0,0){\line(1,0){36}}
	\put(36,0){\line(1,1){36}}
	\put(72,36){\line(1,-1){36}}
	\put(0,4){\line(1,0){36}}
	\put(36,4){\line(1,1){36}}
	\put(72,40){\line(1,-1){36}}
	\put(-6,-25){\scriptsize$#1$}
	\put(30,-25){\scriptsize$#2$}
	\put(66,-25){\scriptsize$#3$}
	\put(102,-25){\scriptsize$#4$}
\end{picture}}
